Decision Based Uncertainty Propagation Using Adaptive Gaussian Mixtures

Given a decision process based on the approximate probability density function returned by a data assimilation algorithm, an interaction level between the decision making level and the data assimilation level is designed to incorporate the information held by the decision maker into the data assimilation process. Here the information held by the decision maker is a loss function at a decision time which maps the state space onto real numbers which represent the threat associated with different possible outcomes or states. The new probability density function obtained will address the region of interest, the area in the state space with the highest threat, and will provide overall a better approximation to the true conditional probability density function within it. The approximation used for the probability density function is a Gaussian mixture and a numerical example is presented to illustrate the concept.

==> update1.tex <==
For discrete-time case, consider the following nonlinear dynamic system with uncertain initial conditions given by the Gaussian mixture pdf \eqref{gauss_sum} and discrete measurement model:
%
\begin{align}
\mathbf{x}_{k+1} &= \mathbf{f}(t_k, \mathbf{x}_k) + \bm{\eta}_k \label{state_eq_discrete} \\
\textbf{z}_k &= \textbf{h}(t_k,\textbf{x}_k) + \textbf{v}_k \label{meas_eq_discrete}
\end{align}
%
and a set of $k$ observations, $\textbf{Z}_k = \{ \textbf{z}_i ~|~ i=1\ldots k\}$. Here $\bm{\eta}_k \sim \mathcal{N}(\mathbf{0}, \mathbf{Q}_k)$ represents the process noise. The same assumptions on process and measurement noise are made as in the continuous-time case.

The Gaussian Sum Filter used to propagate the conditional pdf, $\hat{p}(t_k, \mathbf{x}_k | \mathbf{Z}_k)$ is very similar with the filter used in continuous-time case, except the time-update step which is given by:
%
\begin{align}
\bm{\mu}_{k+1|k}^i &= \mathbf{f}(k, \bm{\mu}_{k|k}^i) \label{discrete_mu} \\
%
\mathbf{P}_{k+1|k}^i &= \textbf{A}_k^i \mathbf{P}_{k|k}^i (\textbf{A}_k^i)^T + \textbf{Q}_k  \label{discrete_P} \\
%
\textrm{where} \quad \textbf{A}_k^i &= \frac{\partial \mathbf{f}(k, \textbf{x}_k)} {\partial \textbf{x}_k}  \bigg|_{\textbf{x}_k = \bm{\mu}_{k|k}^i} \\
%
w_{k+1|k}^i &= w_{k|k}^i \label{weights_forecast_discrete}
\end{align}

Since the measurement model is also discrete, the same measurement update step as in the previous section, Eq.\eqref{meas_ini}-\eqref{meas_fin}, holds also for discrete-time dynamical systems.

The same argument is made here regarding the forecast weights, Eq.\eqref{weights_forecast_discrete}, that are not changed during propagation. A better approximation of the forecast pdf and a more accurate estimate may be obtained by updating these weights.

The true conditional pdf, $p(t_{k+1}, \mathbf{x}_{k+1} | \mathbf{Z}_k)$ is given by the Chapman-Kolmogorov equation:

\footnotesize\begin{align}
p(t_{k+1}, \mathbf{x}_{k+1} | \mathbf{Z}_k) &= \int p(t_{k+1}, \mathbf{x}_{k+1} | t_k, \mathbf{x}_k ) p(t_k, \mathbf{x}_k | \mathbf{Z}_k) \mathrm{d}\mathbf{x}_k \label{CKE}
\end{align}\normalsize

The new weights may be obtained in the least square sense to minimize the following integral square difference between the true conditional density function and its approximation:

\small\begin{align}
\min_{w_{k+1|k}^i} ~&~ \frac{1}{2} \int \big| p(t_{k+1}, \textbf{x}_{k+1}|\mathbf{Z}_k) - \hat{p}(t_{k+1}, \textbf{x}_{k+1}|\mathbf{Z}_k) \big|^2 \textrm{d}\textbf{x}_{k+1} \label{cost_function}  \\
%
\textrm{s.t.} ~&~ \sum^{N}_{i=1} w_{k+1|k}^i = 1 \nonumber \\
&~ w_{k+1|k}^i \ge 0, \quad i=1,\cdots,N \nonumber
\end{align}\normalsize

Here, no \textsl{a priori} structure is used for the true conditional density function $p(t_{k+1}, \textbf{x}_{k+1}|\mathbf{Z}_k)$, it is completely unknown.

The final formulation of the optimization \eqref{cost_function} may be posed in the quadratic programming framework\cite{Terejanu2007} and solved using readily available solvers:
%
\begin{align}
\min_{\mathbf{w}_{k+1|k}} ~&~ \frac{1}{2} \textbf{w}_{k+1|k}^T \textbf{M} \textbf{w}_{k+1|k} - \textbf{w}_{k+1|k}^T \textbf{N} \textbf{w}_{k|k} \label{main_cost_func} \\
%
\textrm{s.t.} ~&~ \textbf{1}_{N\times1}^T \textbf{w}_{k+1|k} = 1 \nonumber \\
%
~&~ \textbf{w}_{k+1|k} \ge \textbf{0}_{N\times1}  \nonumber
\end{align}
\begin{table}[h]
\renewcommand{\arraystretch}{2}
\begin{center}
\caption{GSF3 - Forecast Weights Update Method II - Discrete-Time Dynamical Systems}
\label{GSF3}
\begin{tabular}{|l|}
\hline
\textbf{Discrete-time nonlinear dynamics:} \\
\hline
$\mathbf{x}_{k+1} = \mathbf{f}(t_k, \mathbf{x}_k) + \bm{\eta}_k$ \\
\hline
\textbf{Discrete-time measurement model:} \\
\hline
$\textbf{z}_k = \textbf{h}(t_k,\textbf{x}_k) + \textbf{v}_k$ \\
\hline
\textbf{Propagation:} \\
\hline
$\bm{\mu}_{k+1|k}^i = \mathbf{f}(k, \bm{\mu}_{k|k}^i)$ \\
%
$\mathbf{P}_{k+1|k}^i = \textbf{A}_k^i \mathbf{P}_{k|k}^i (\textbf{A}_k^i)^T + \textbf{Q}_k$ \\
%
$\textbf{A}_k^i = \frac{\partial \mathbf{f}(k, \textbf{x}_k)} {\partial \textbf{x}_k}  \bigg|_{\textbf{x}_k = \bm{\mu}_{k|k}^i}$ \\
%
$\mathbf{w}_{k+1|k} = \arg\min\limits_{\mathbf{w}_{k+1|k}} ~~ \frac{1}{2} \textbf{w}_{k+1|k}^T \textbf{M} \textbf{w}_{k+1|k} - \textbf{w}_{k+1|k}^T \textbf{N} \textbf{w}_{k|k}$ \\
%
\hspace{.53in}$\textrm{subject to} \quad \textbf{1}_{N\times1}^T \mathbf{w}_{k+1|k} = 1$ \\
%
\hspace{1.1in}$\textbf{w}_{k+1|k} \ge \textbf{0}_{N\times1}$ \\
\hline
\textbf{Measurement Update:} \\
\hline
$\bm{\mu}_{k+1|k+1}^i = \bm{\mu}_{k+1|k}^i + \mathbf{K}_k^i \left( \mathbf{z}_k - \mathbf{h}(t, \bm{\mu}_{k+1|k}^i) \right)$ \\
%
$\mathbf{P}_{k+1|k+1}^i = \left( \mathbf{I} - \mathbf{K}_k^i \mathbf{H}_k^i \right) \mathbf{P}_{k+1|k}^i$ \\
%
$\textbf{H}_k^i = \frac{\partial \mathbf{h}(t, \textbf{x}_k)} {\partial \textbf{x}_k} \bigg|_{\textbf{x}_k = \bm{\mu}_{k+1|k}^i}$ \\
%
$\mathbf{K}_k^i = \mathbf{P}_{k+1|k}^i \mathbf{H}_k^i \left( \mathbf{H}_k^i \mathbf{P}_{k+1|k}^i (\mathbf{H}_k^i)^t + \mathbf{R}_k \right)^{-1}$ \\
%
$w_{k+1|k+1}^i = \frac{w_{k+1|k}^i \beta_k^i}{\sum^{N}_{i=1} w_{k+1|k}^i \beta_k^i}$ \\
%
$\beta_k^i = \mathcal{N}\left(\mathbf{z}_k - \mathbf{h}(t, \bm{\mu}_{k+1|k}^i), ~ \mathbf{H}_k^i \mathbf{P}_{k+1|k}^i (\mathbf{H}_k^i)^t + \mathbf{R}_k \right)$ \\
\hline
\end{tabular}
\end{center}
\end{table}


This optimization problem will replace Eq.\eqref{weights_forecast_discrete}. Here $\textbf{1}_{N\times1}$ is a vector of ones and $\textbf{0}_{N\times1}$ is a vector of zeros, $\textbf{w}_{k+1|k} = [w_{k+1|k}^1 ~ w_{k+1|k}^2 ~ \ldots ~ w_{k+1|k}^N]^T$ is the vector of forecast weights, $\textbf{w}_{k|k} = [w_{k|k}^1 ~ w_{k|k}^2 ~ \ldots ~ w_{k|k}^N]^T$ is the prior weight vector, and $\textbf{M}_{N\times N}$ is a symmetric matrix given by:
%
\begin{align}
\textbf{M}_{N\times N} &= \int \mathbf{\mathfrak{M}}(\textbf{x}_{k+1}) \mathbf{\mathfrak{M}}^T(\textbf{x}_{k+1}) \textrm{d}\textbf{x}_{k+1} \label{cont_matrix}
\end{align}
%
where $\mathbf{\mathfrak{M}}$ is a $N \times 1$ vector that contains all the propagated  Gaussian components at time $k+1$:
%
\begin{align}
\mathbf{\mathfrak{M}}(\textbf{x}_{k+1}) &= \left[ \begin{array}{r}
\mathcal{N}(\textbf{x}_{k+1} ~|~ \bm{\mu}_{k+1|k}^1, \mathbf{P}_{k+1|k}^1) \\ \mathcal{N}(\textbf{x}_{k+1} ~|~ \bm{\mu}_{k+1|k}^2, \mathbf{P}_{k+1|k}^2) \\
\ldots \hspace{0.6in}\\
\mathcal{N}(\textbf{x}_{k+1} ~|~ \bm{\mu}_{k+1|k}^N, \mathbf{P}_{k+1|k}^N)
\end{array} \right]
\end{align}

Thus, the components of matrix $\textbf{M}$ are easily given by the product rule of two Gaussian density functions which yields another Gaussian density function. By integrating the product we are left only with the normalization constant:
%
\small\begin{align}
m_{ij} =&  \left|2\pi(\mathbf{P}_{k+1|k}^i+\mathbf{P}_{k+1|k}^j)\right|^{-1/2}  \textrm{exp}\left[ -\frac{1}{2}(\bm{\mu}_{k+1|k}^i-\bm{\mu}_{k+1|k}^j)^T \right. \nonumber \\
%
&\left.\times(\mathbf{P}_{k+1|k}^i+\mathbf{P}_{k+1|k}^j)^{-1}(\bm{\mu}_{k+1|k}^i-\bm{\mu}_{k+1|k}^j)\right] \\
%
m_{ii} =& \left|4\pi\mathbf{P}_{k+1|k}^i\right|^{-1/2}
\end{align}\normalsize

Using Chapman-Kolmogorov equation \eqref{CKE}, we are able to derive the following expressions for the elements of matrix $\textbf{N}_{N\times N}$ from  Eq.\ref{main_cost_func}:

\small\begin{align}
n_{ij} =& \int \mathcal{N}(\textbf{f}(t_k, \textbf{x}_k) ~|~ \bm{\mu}_{k+1|k}^i, \mathbf{P}_{k+1|k}^i + \mathbf{Q}_k) \nonumber\\
&\times \mathcal{N}(\textbf{x}_k ~|~ \bm{\mu}_{k|k}^j, \mathbf{P}_{k|k}^j) ~ \textrm{d}\textbf{x}_k \label{integral} \\
%
=& \textrm{E}_{\mathcal{N}(\textbf{x}_k | \bm{\mu}_{k|k}^j, \mathbf{P}_{k|k}^j)} \left[\mathcal{N}(\textbf{f}(t_k, \textbf{x}_k) \big| \bm{\mu}_{k+1|k}^i, \mathbf{P}_{k+1|k}^i + \mathbf{Q}_k)\right] \label{expectation}
\end{align}\normalsize

The expectations \eqref{expectation} may be computed using Gaussian Quadrature, Monte Carlo integration or Unscented Transformation \cite{Julier2004}. Let the weighted sigma points $\left\{\mathcal{W}_k^l, \mathcal{X}_k^l \right\}$, where $l=1\ldots L$, sample the a posteriori normal distribution $\mathcal{N}\left(\textbf{x}_k | \bm{\mu}_{k|k}^j, \mathbf{P}_{k|k}^j\right)$. The transformed sigma points $\left\{\mathcal{W}_k^l, \mathcal{X}_{k+1}^l \right\}$ are obtained by using the Unscented Transformation \cite{Julier2004}. Thus we can numerically compute $n_{ij}$ using the following relation:
%
\begin{align}
n_{ij} =& \sum^{L}_{l=1} \mathcal{W}_k^l \mathcal{N}(\mathcal{X}_{k+1}^l \big| \bm{\mu}_{k+1|k}^i, \mathbf{P}_{k+1|k}^i) \label{approx}
\end{align}
%
While in lower dimensions the unscented transformation is mostly equivalent with Gaussian quadrature, in higher dimensions the unscented transformation is computational more appealing in evaluating integrals since the number of points grows only linearly with the number of dimensions. However, this comes with a loss in accuracy \cite{Honkela2004}, hence the need for a larger number of points \cite{Wu2004} to capture additional information.

In the case of linear transformation, $\mathbf{f}(t_k, \cdot) = \mathbf{F}_k$, and by manipulating Eq.\eqref{integral}, $m_{ij} = n_{ij}$, yielding $\textbf{M} = \textbf{N}$, hence no change will occur to the weights. However, the numerical approximations \eqref{approx} made in computing the expectations \eqref{expectation} may not give a perfect match between the two matrices, thus deteriorating the overall results in this case. Hence, such an update scheme may be recommended only for nonlinear systems.

The summary of the Gaussian Sum Filter with forecast weight update for the discrete-time nonlinear dynamical systems is presented in Table~\ref{GSF3}.
%


==> update2.tex <==
In this section, we summarize a recently developed method to update the weights of different components of the Gaussian mixture \eqref{gaussappr} during propagation. It can be shown that the true state probability density function, $p(t, \mathbf{x}(t)|\mathbf{Z}_k)$, satisfies the FPKE~\eqref{fpke} between observations \cite{Jazwinski1970}, which is a second order partial differential equation in $p(t, \mathbf{x}(t)|\mathbf{Z}_k)$.
%
\begin{equation} \label{fpke}
\frac{\partial}{\partial t}p(t, \mathbf{x}|\mathbf{Z}_k) = \mathcal{L_{FP}}p(t, \mathbf{x}|\mathbf{Z}_k)
\end{equation}

The main idea is to modify the weights of the approximate conditional pdf given by  Gaussian mixture \eqref{gaussappr}, $\hat{p}(t, \mathbf{x}|\mathbf{Z}_k)$, such that it satisfies the FPKE \eqref{fpke}.

The FPKE error can be used as a feedback to update the weights of different Gaussian components in the mixture pdf. In another words, we seek to minimize the FPKE error under the assumption \eqref{gaussappr}, \eqref{meanprop} and~\eqref{covprop}.

The substitution \eqref{gaussappr} in \eqref{fpke} leads to
%
\begin{align}
e(t, \mathbf{x}) &= \frac{\partial \hat{p}(t, \mathbf{x}|\mathbf{Z}_k)}{\partial t}-\mathcal{L_{FP}}(\hat{p}(t, \mathbf{x}|\mathbf{Z}_k))\\\label{fpkerror}
%
\mathcal{L_{FP}} &= \left[-\sum_{i=1}^{n}{\frac{\partial \mathrm{D}_i^{(1)} (t, \mathbf{x})} {\partial x_i} + \sum_{i=1}^{n}\sum_{j=1}^{n}}\frac{\partial^2 \mathrm{D}_{ij}^{(2)}(t, \mathbf{x})}{\partial x_i\partial x_j} \right] \\
%
\label{drift}\mathrm{D}^{(1)}(t, \mathbf{x}) &= \mathbf{f}(t, \mathbf{x}) + \frac{1}{2} \frac{\partial \mathbf{g}(t, \mathbf{x})}{\partial \mathbf{x}} \mathbf{Q} \mathbf{g} (t, \mathbf{x})&&\\
%
\label{diffusion} \mathrm{D}^{(2)}(t, \mathbf{x}) &= \frac{1}{2} \mathbf{g}(t, \mathbf{x}) \mathbf{Q} \mathbf{g}^\mathrm{T}(t, \mathbf{x})&&
\end{align}
%
where $\mathcal{L_{FP}(\cdot)}$ is the so called Fokker-Planck operator, and,
%
\footnotesize\begin{align}\label{timederiv}
\frac{\partial \hat{p}(t, \mathbf{x}|\mathbf{Z}_k)}{\partial t} &= \sum\limits_{i=1}^N w^i_{t|k}\left[ \frac{\partial p_{g_i}}{\partial \bm{\mu}^i_{t|k}}^T\dot{\bm{\mu}}^i_{t|k}+ \sum\limits_{j=1}^{n}\sum\limits_{k=1}^{n}\frac{\partial p_{g_i}}{\partial P^{i,jk}_{t|k}}\dot{P}^{i,jk}_{t|k} \right]
\end{align}\normalsize
%
where $P^{i,jk}_{t|k}$ is the $jk^{th}$ element of the $i^{th}$ covariance matrix $\mathbf{P}^i_{t|k}$. Further, substitution of \eqref{drift} and \eqref{diffusion} along with  \eqref{timederiv} in \eqref{fpkerror} leads to
%
\begin{equation}\label{linerr}
e(t, \mathbf{x}) = \sum\limits_{i=1}^{N}w^i_{t|k} \mathbf{\mathfrak{L}}_i(t, \mathbf{x}) = \mathbf{\mathfrak{L}}^T \mathbf{w}_{t|k}
\end{equation}
%
where $\mathbf{w}_{t|k}$ is a $N\times 1$ vector of Gaussian weights, and $\mathbf{\mathfrak{L}}_i$ is given by
%
\begin{align}
\mathbf{\mathfrak{L}}_i(t, \mathbf{x})&= \left[\frac{\partial p_{g_i}}{\partial\bm{\mu}^i_{t|k}}^T \textbf{f}(t,\bm{\mu}^i_{t|k}) + \sum\limits_{j=1}^{n}\sum\limits_{k=1}^{n}\frac{\partial p_{g_i}}{\partial P^{i,jk}_{t|k}}\dot{P}^{i,jk}_{t|k}\right. \nonumber\\
%
&\left. + \sum\limits_{j=1}^n\left(f_j(t, \textbf{x})\frac{\partial p_{g_i}}{\partial x_j} + p_{g_i}\frac{\partial f_j(t, \mathbf{x})}{\partial x_j}\right.\right. \nonumber\\
%
&\left.\left. + \frac{1}{2}\frac{\partial d^{(1)}_j(t,\mathbf{x})p_{g_i}}{\partial x_j} - \frac{1}{2}\sum\limits_{k=1}^n\frac{\partial^2d^{(2)}_{jk}(t,\mathbf{x})p_{g_i}}{x_jx_k} \right)\right]
\end{align}
%
$d^{(1)}(t,\mathbf{x})$ and $d^{(2)}(t,\mathbf{x})$ are given as:
%
\begin{eqnarray}
&&d^{(1)}(t,\mathbf{x}) = \frac{1}{2}\frac{\partial \mathbf{g}(t,\mathbf{x})}{\partial\mathbf{x}}\mathbf{Q}\mathbf{g}(t,\mathbf{x})\\
%
&&d^{(2)}(t,\mathbf{x}) = \frac{1}{2}\mathbf{g}(t,\mathbf{x})\mathbf{Q}\mathbf{g}^T(t,\mathbf{x})
\end{eqnarray}
%
Further, different derivatives in the above equation can be computed using the following analytical formulas:
%
\small\begin{align}
\frac{\partial{p_{g_i}}}{\partial{\bm{\mu}^i_{t|k}}} &= (\mathbf{P}^i_{t|k})^{-1}\left(\mathbf{x}-\bm{\mu}^i_{t|k}\right)p_{g_i} \nonumber\\
%
\frac{\partial{p_{g_i}}}{\partial{\mathbf{P}^i_{t|k}}} &= \frac{p_{g_i}}{2}(\mathbf{P}^i_{t|k})^{-1}\left[\left(\mathbf{x}-\bm{\mu}^i_{t|k}\right)\left(\mathbf{x}-\bm{\mu}^i_{t|k}\right)^T(\mathbf{P}^i_{t|k})^{-1} - \mathbf{I} \right] \nonumber\\
%
\frac{\partial{p_{g_i}}}{\partial{\mathbf{x}}} &= -(\mathbf{P}^i_{t|k})^{-1}\left(\mathbf{x}-\bm{\mu}^i_{t|k}\right)p_{g_i} \nonumber\\
%
\frac{\partial^2{p_{g_i}}}{\partial{\mathbf{x}\mathbf{x}^T}} &= -(\mathbf{P}^i_{t|k})^{-1}\left[\mathbf{I}+\left(\mathbf{x}-\bm{\mu}^i_{t|k}\right)\frac{\partial{p_{g_i}}}{\partial{\mathbf{x}}}^T\right]p_{g_i} \nonumber
\end{align}\normalsize
%
Now, at a given time instant, after propagating the mean, $\bm{\mu}^i_{t|k}$ and the covariance, $\mathbf{P}^i_{t|k}$, of individual Gaussian elements using \eqref{meanprop} and \eqref{covprop}, we seek to update weights by minimizing the FPE equation error over some volume of interest $V$:
%
\begin{align}
\min\limits_{w^i_{t|k}} ~&~ \frac{1}{2} \int\limits_V e^2(t, \mathbf{x}) \textrm{d}\mathbf{x} + \sum\limits_{i=1}^{N}(w^i_{t|k}-w^i_{k|k})^2\\
%
\textrm{s.t} ~&~ \sum\limits_{i=1}^{N} w^i_{t|k} = 1 \nonumber \\
%
&~ w^i_{t|k}\ge 0,\quad i=1,\cdots,N \nonumber
\end{align}
%
Here, the second term in the cost function is introduced to penalize large variations in the weights between two time steps. Since, FPKE error \eqref{linerr} is linear in Gaussian weights, $w^i_{t|k}$, hence, the aforementioned problem can be written as a quadratic programming problem.
%
\begin{align}\label{quad1}
\min\limits_{\mathbf{w}_{t|k}} ~&~ \frac{1}{2} \mathbf{w}_{t|k}^T\mathbf{L}\mathbf{w}_{t|k} + (\mathbf{w}_{t|k}-\mathbf{w}_{k|k})^T(\mathbf{w}_{t|k}-\mathbf{w}_{k|k}) \\
%
\textrm{s.t} ~&~ \textbf{1}_{N\times1}^T \mathbf{w}_{t|k} = 1 \nonumber \\
%
&~ \textbf{w}_{t|k} \ge \textbf{0}_{N\times1}  \nonumber
\end{align}
%
where $\textbf{1}_{N\times1}$ is a vector of ones, $\textbf{0}_{N\times1}$ is a vector of zeros and $\mathbf{L}$ is given by
%
\begin{align} \label{Lmatrix}
\mathbf{L} &= \int\limits_V\mathbf{\mathfrak{L}}(\mathbf{x})\mathbf{\mathfrak{L}}^T(\mathbf{x})\mathrm{d}\mathbf{x} \nonumber \\
&= \left[\begin{array}{cccc} \int\limits_V\mathbf{\mathfrak{L}}_1\mathbf{\mathfrak{L}}_{1}\textrm{d}\mathbf{x} & \int\limits_V\mathbf{\mathfrak{L}}_2\mathbf{\mathfrak{L}}_{1}\textrm{d}\mathbf{x} & \cdots & \int\limits_V\mathbf{\mathfrak{L}}_N\mathbf{\mathfrak{L}}_{1}\textrm{d}\mathbf{x} \\
%
\int\limits_V\mathbf{\mathfrak{L}}_1\mathbf{\mathfrak{L}}_{2}\textrm{d}\mathbf{x} & \int\limits_V\mathbf{\mathfrak{L}}_2\mathbf{\mathfrak{L}}_{2}\textrm{d}\mathbf{x} & \cdots & \int\limits_V\mathbf{\mathfrak{L}}_N\mathbf{\mathfrak{L}}_{2}\textrm{d}\mathbf{x} \\
%
\vdots & & \ddots& \vdots \\
%
\int\limits_V\mathbf{\mathfrak{L}}_1\mathbf{\mathfrak{L}}_{N}\textrm{d}\mathbf{x} & \int\limits_V\mathbf{\mathfrak{L}}_2\mathbf{\mathfrak{L}}_{N}\textrm{d}\mathbf{x} & \cdots & \int\limits_V\mathbf{\mathfrak{L}}_N\mathbf{\mathfrak{L}}_{N}\textrm{d}\mathbf{x}\\
\end{array}\right]
\end{align}

Notice, to carry out this minimization, we need to evaluate integrals involving Gaussian pdfs over volume $V$ which can be computed exactly for polynomial nonlinearity and in general can be approximated by the Gaussian quadrature method.

The minimization problem \eqref{quad1} will substitute the Eq. \eqref{forecast_weights} whenever an estimate has to be computed, even between measurements.

The summary of the Gaussian Sum Filter with forecast weight update for the continuous-time nonlinear dynamical systems and discrete measurement model is presented in Table~\ref{GSF2}.
%
\begin{table}[htbp]
\renewcommand{\arraystretch}{2}
\begin{center}
\caption{GSF2 - Forecast Weights Update Method I - Continuous-Time Dynamical Systems}
\label{GSF2}
\begin{tabular}{|l|}
\hline
\textbf{Continuous-time nonlinear dynamics:} \\
\hline
$\dot{\mathbf{x}}(t) = \mathbf{f}(t, \mathbf{x}(t)) + \mathbf{g}(t, \mathbf{x}(t))  \Gamma(t)$ \\
\hline
\textbf{Discrete-time measurement model:} \\
\hline
$\textbf{z}_k = \textbf{h}(t_k,\textbf{x}_k) + \textbf{v}_k$ \\
\hline
\textbf{Propagation:} \\
\hline
$\dot{\bm{\mu}}_{t|k}^i = \mathbf{f}(t,\bm{\mu}_{t|k}^i)$ \\
%
$\dot{\mathbf{P}}_{t|k}^i = \mathbf{A}_{t|k}^i \mathbf{P}_{t|k}^i+\mathbf{P}_{t|k}^i (\mathbf{A}_{t|k}^i)^T+\mathbf{g}(t, \bm{\mu}_{t|k}^i) \mathbf{Q} \mathbf{g}^T(t, \bm{\mu}_{t|k}^i)$ \\
%
$\textbf{A}_{t|k}^i = \frac{\partial \mathbf{f}(t, \textbf{x}(t))} {\partial \mathbf{x}(t)} \bigg|_{\textbf{x}(t) = \bm{\mu}_{t|k}^i}$ \\
%
$\mathbf{w}_{t|k} = \arg\min\limits_{\mathbf{w}_{t|k}} ~~ \frac{1}{2} \mathbf{w}_{t|k}^T\mathbf{L}\mathbf{w}_{t|k} + (\mathbf{w}_{t|k}-\mathbf{w}_{k|k})^T(\mathbf{w}_{t|k}-\mathbf{w}_{k|k})$ \\
%
\hspace{.4in}$\textrm{subject to} \quad \textbf{1}_{N\times1}^T \mathbf{w}_{t|k} = 1$ \\
%
\hspace{.95in}$\textbf{w}_{t|k} \ge \textbf{0}_{N\times1}$ \\
\hline
\textbf{Measurement-Update:} \\
\hline
$\bm{\mu}_{k+1|k+1}^i = \bm{\mu}_{k+1|k}^i + \mathbf{K}_k^i \left( \mathbf{z}_k - \mathbf{h}(t, \bm{\mu}_{k+1|k}^i) \right)$ \\
%
$\mathbf{P}_{k+1|k+1}^i = \left( \mathbf{I} - \mathbf{K}_k^i \mathbf{H}_k^i \right) \mathbf{P}_{k+1|k}^i$ \\
%
$\mathbf{H}_k^i = \frac{\partial \mathbf{h}(t, \textbf{x}_k)} {\partial \textbf{x}_k} \bigg|_{\mathbf{x}_k = \bm{\mu}_{k+1|k}^i}$ \\
%
$\mathbf{K}_k^i = \mathbf{P}_{k+1|k}^i \mathbf{H}_k^i \left( \mathbf{H}_k^i \mathbf{P}_{k+1|k}^i (\mathbf{H}_k^i)^t + \mathbf{R}_k \right)^{-1}$ \\
%
$w_{k+1|k+1}^i = \frac{w_{k+1|k}^i \beta_k^i}{\sum^{N}_{i=1} w_{k+1|k}^i \beta_k^i}$ \\
%
$\beta_k^i = \mathcal{N}\left(\mathbf{z}_k - \mathbf{h}(t, \bm{\mu}_{k+1|k}^i), ~ \mathbf{H}_k^i \mathbf{P}_{k+1|k}^i (\mathbf{H}_k^i)^t + \mathbf{R}_k \right)$ \\
\hline
\end{tabular}
\end{center}
\end{table}


